Safe Adaptive Switching among Dynamical Movement Primitives: Application to 3D Limit-Cycle Walkers

Complex motions for robots are frequently generated by switching among a collection of individual movement primitives. We use this approach to formulate robot motion plans as sequences of primitives to be executed one after the other. When dealing with dynamical movement primitives, besides accomplishing the high-level objective, planners must also reason about the effect of the plan's execution on the safety of the platform. This task becomes more daunting in the presence of disturbances, such as external forces. To alleviate this issue, we present a framework that builds on rigorous control-theoretic tools to generate safely-executable motion plans for externally excited robotic systems. Our framework is illustrated on a 3D limit-cycle gait bipedal robot that adapts its walking pattern to persistent external forcing.

==> leftovers.tex <==
%Least square error minimization is performed to fit polynomials to these data points. 
%The AWAFs $\tilde{\mathcal{A}}_p(z)$ estimated in Section~\ref{subsec:AWAF} for the gait primitives $\mathcal{G}_1$ for straight walking, $\mathcal{G}_2$ for turning by $45^o$, and $\mathcal{G}_3$ for turning by $-45^o$, will be used here. The AWAFs are fed to the planner presented in Table~\ref{tab:RRT} to generate motion plans in two environments cluttered by obstacles.

%The planner presented in Table~\ref{tab:RRT} using AWAFs is used to generate motion plans in two environments. 
%AWAF is used to generate a motion plan for two environments using the RRT algorithm in Section~\ref{sec:RRT}. The environment shown in Fig.~\ref{fig:greg_map} is borrowed from \cite{gregg-planning2012} and \cite{motahar2016composing} where the final drift error for a plan with the same initial position and goal is 2.59 m and 1.20 m, respectively. Using our planning approach the drift error is only 3.40 mm. To demonstrate that our planner can work in tight environments as well, we plan the motion of our biped for the environment shown in Fig.~\ref{fig:narrow_map} borrowed from \cite{motahar2016composing}. The initial position and orientation of the biped and the goal position is chosen similar to \cite{motahar2016composing} where the final drift was 6.3 cm. The drift for the execution of our plan in Fig.~\ref{fig:narrow_map} is only 0.65 mm.


%The order of the polynomials was increased till a substantial improvement in the fit was observed. 
%$(\delta X_p(z),\delta Y_p(z))$, we use $l_p(z) = \|(\delta X_p(z),\delta Y_p(z))\|$, and $s_p(z) = \arctan(\delta Y_p(z) / \delta X_p(z))$,
%\begin{itemize}
%\item $l_p(z) = \|\delta \mathrm{cm}_p^z(z)\|$, and
%\item $s_p(z) = \arctan(\delta \mathrm{cm}_{p,Y}^z(z) / \delta \mathrm{cm}_{p,X}^z(z))$,
%\end{itemize}   
%as a surrogate for $(\delta X_p(z),\delta Y_p(z))$.
%
%In this section we extract the AWAFs for a particular set of gait primitives and then compare their effectiveness against NWAs. 
%
%The primitive $\mathcal{G}_1$ corresponds to the biped walking straight in the current heading direction. The biped turns by $45^o$  and $-45^o$ under the effect of $\mathcal{G}_2$ and $\mathcal{G}_3$, respectively. 
%With $\kappa$ available to us we compute $\omega_1(\kappa)$, $\omega_2(\kappa)$, and $\omega_3(\kappa)$ and use them to compute the corresponding $r_p$ using \eqref{eq:rp} which takes the form 
%$r_p = \sqrt{\frac{\omega_p(\kappa)}{\lambda_{\min}(S_p)}}$
%$r_p = \sqrt{\omega_p(\kappa)/\lambda_{\min}(S_p)}$.
%The set $\mathcal{B}$ is meshed as shown in Fig.~\ref{fig:mesh} overlaid on top of $\overline{\mathcal{M}}(\kappa)$. 

%We choose our exponential Lyapunov function $V_p(z)$ to have a quadratic form, i.e., $V_p(z)=z^{\rm T} S_p z$ where $S_p$ is the solution of the discrete Lyapunov equation for the linearization of \eqref{eq:zd-system}. A sum-of-squares (SOS) \cite{tedrake2010} verification is performed using $V_p(z)$ to obtain positively invariant sublevel sets for applying Theorem~\ref{thm:switched}. The analysis presented in \cite[Section~V-C.]{motahar2016composing} establishes that any plan with 
%Theorem~\ref{thm:switched} is applied to \eqref{eq:switched-system} in \cite[Section~V-C]{motahar2016composing} to show that $N_{\rm d}\geq 1$ is sufficient to guarantee stable execution of the plan for the biped under consideration in this paper; see Fig.~\ref{fig:model}. 

%We begin by finding balls that enclose each $\mathcal{M}_p(\kappa)$ and are centered about the corresponding $z_p^*$. From the definition of $\mathcal{M}_p(\kappa)$ we have $V_p(z)\leq \omega_p(\kappa)$. Using the first inequality of \eqref{eq:V_1} we get
%%eq
%\begin{equation}\label{eq:rp}
%\|z-z_p^*\| \leq \chi_{p,1}^{-1}(\omega_p(\kappa))=:r_p\enspace.
%\end{equation}
%%eq
%Without loss of generality, we assume that the ball which encloses the entire compact set $\overline{\mathcal{M}}(\kappa)$ is centered at $z_0^*$. The radius of that ball can be chosen as
%%eq
%\begin{equation}\label{eq:R}
%R := \max_{p\in\mathcal{P}} \{ \|z_p^*-z_0^*\| + r_p\}
%\end{equation}
%%eq
%where $r_p$ is defined in \eqref{eq:rp}. Next, define the set\footnote{Notation: Euclidean norm denoted by $\|\cdot\|$; p-$\infty$ norm denoted by $\|\cdot\|_\infty$.}
%%eq
%\begin{equation}\label{eq:mesh-set}
%\mathcal{B}:=\{z\in\mathcal{D}~:~\|z-z_0^*\|_\infty \leq R \}
%\end{equation}
%%eq
%which we will mesh to fit polynomials and obtain approximations of the reduced Poincar\'e map and WAF. The low dimensionality of $z$ makes this computationally feasible.


% $\tilde{\rho}_p(z)$, $\delta \tilde{q}_{1,p}(z)$, $\tilde{l}_p(z)$, and $\tilde{s}_p(z)$ for each $p\in\mathcal{P}$. The AWAFs defined as $\tilde{\mathcal{A}}_p(z):=(\tilde{\rho}_p(z),\delta \tilde{q}_{1,p}(z),\tilde{l}_p(z),\tilde{s}_p(z))$ are made available to the planner as actions.

 
%Instead of approximating each component of $(\delta X_p(z),\delta Y_p(z))$, we use $l_p(z) = \|(\delta X_p(z),\delta Y_p(z))\|$, and $s_p(z) = \arctan(\delta Y_p(z) / \delta X_p(z))$,
%%\begin{itemize}
%%\item $l_p(z) = \|\delta \mathrm{cm}_p^z(z)\|$, and
%%\item $s_p(z) = \arctan(\delta \mathrm{cm}_{p,Y}^z(z) / \delta \mathrm{cm}_{p,X}^z(z))$,
%%\end{itemize}   
%as a surrogate for $(\delta X_p(z),\delta Y_p(z))$. To obtain the AWAF we need a mesh on a subset of $\mathcal{S}\cap\mathcal{Z}$ within which $\rho_p(z)$ is well-defined for all $p\in\mathcal{P}$. We can do better than that by using Theorem~\ref{thm:switched} as illustrated in the remark below.

%where the planner requires a change from one action $\mathcal{A}_p(z_p^*)$  to subsequent one $\mathcal{A}_q(z_q^*)$. If $p \neq q$ the state at the end of the previous action $z_p^*$ differs from the state $z_q^*$ the corresponds to the next action.
%The state of the system at the beginning of the plan is $z=z_1^*$. If at the end, the planner does not change primitive, the state $z$ will be aligned with the state of the action, namely $z_1^*$ causing no drift. However, if the planner suggests the change of action the state $z$ which is $z_1^*$ is going to be different from $z_2^*$. As a result at the end of the execution, the planner will be thinking that the system advanced by $\{ \delta q_{1,p}(z_2^*),\delta X_2(z_2^*),\delta Y_2(z_2^*) \}$ corresponding to the discrete action $\mathcal{A}_2(z_2^*)$ 
%The cause of the drift is illustrated in Fig.~\ref{fig:tree_error} for the gait primitives $\mathcal{G}_1$ and $\mathcal{G}_2$ that correspond to straight walking and turning left, respectively. It is assumed that the state of the biped at a corresponds to the fixed point for walking straight, i.e., $z_a = z_1^*$. The biped walks straight from a to b and no disagreement between the actual path and the NWA is observed as $z_a$ corresponds to the fixed point of the gait primitive applied. At b the planner decides to turn left, the state $z_b = z_1^*$ is not aligned with the fixed point $z_2^*$. Thus, the biped's motion would correspond to $\mathcal{A}_2(z_1^*)$ taking it to c, however, the NWA would be $\mathcal{A}_2(z_2^*)$ making the planner anticipate the position of the biped as d, resulting in a drift. 
%From Theorem~\ref{thm:switched}, $z[k]\in\overline{\mathcal{M}}(\kappa)$ for all $k\in\mathbb{Z}_+$. Hence, the assumption that the state $z$ is always aligned with the fixed point $z_p^*$ of the corresponding primitive would result in the planner anticipating a different motion than the one executed by the biped. 

%Computing $\rho_p$ involves numerically integrating nonlinear dynamics which would slow down the planning process considerably. Previous work \cite{gregg-planning2012} dealt with this problem by admitting NWAs, $\mathcal{A}_p(z_p^*):=(\delta q_{1,p}(z_p^*),\delta X_p(z_p^*),\delta Y_p(z_p^*))$, as actions to the planner. NWAs are the outputs of \eqref{eq:zd-system} evaluated at the corresponding fixed point $z^*_p$; see \cite[Table~I,II]{gregg-planning2012} and \cite[Table~I]{motahar2016composing}.
%From Theorem~\ref{thm:switched}, $z[k]\in\overline{\mathcal{M}}(\kappa)$ for all $k\in\mathbb{Z}_+$. Hence, the assumption that the state $z$ is always aligned with the fixed point $z_p^*$ of the corresponding primitive would result in the planner anticipating a different motion than the one executed by the biped. This error accumulates over the steps resulting in large drifts by the end of the plan preventing the biped from reaching the goal \cite{gregg-planning2012}. 
%As $z_p^*$ is an exponentially stable fixed point of $\rho_p$, it would take an infinite number of strides for the biped to exactly converge to the limit cycle corresponding to that fixed point after a primitive switch. Hence, the assumption of a \emph{constant} NWA would result in the planner anticipating a different motion than the one executed by the biped. This error accumulates over the steps resulting in large drifts by the end of the plan preventing the biped from reaching the goal \cite{gregg-planning2012}. 
%Similarly, at nodes 3 and 5, the state $x_3$ and $x_5$ are not necessarily the fixed points of the nominal limit-cycle. This causes the planner to predict a motion which is different from the actual behavior of the biped and the error propagates with every step.

%in $\mu(\kappa)$. In fact, as $\kappa\to 0$ then $\mu(\kappa)\to \infty$ which by \eqref{eq:dwell-time} requires $N_{\rm d}\to \infty$. Thus, the improvement in drift by controlling $\kappa$  comes at a price of larger dwell-time bounds which greatly reduces the flexibility of the planner to generate motion plans in environments with `tight' workspaces. Furthermore, even the choice of a small $\kappa$ would not mitigate the drift error substantially as the size of $\overline{\mathcal{M}}(0)\subset\overline{\mathcal{M}}(\kappa)$ for all $\kappa>0$, is governed by how far $z_p^*$ are from each other. Hence, reducing $\kappa$ for controlling drift is not a very effective strategy. 

%Knowledge of the theorem can make the drift smaller as in~\cite{motahar2016composing}, to alimit. But still it cannot be eliminatd. Theorem~\ref{thm:switched} provides a gateway to reduce this drift to a certain extent. By choosing a smaller $\kappa$, the size of $\overline{\mathcal{M}}(\kappa)$ can be reduced resulting in the state $z$ to evolve nearer to the fixed points $z_p^*$. This would mean that the plan generated using NWA would exhibit lower drift as the outputs $\delta q_{1,p}(z)$ and $\delta \mathrm{cm}_p(z)$ are smooth in $z$. 
%Instead, we will use the knowledge that we are trapped in $\overline{\mathcal{M}}(\kappa)$ to obtain \emph{approximate walking arc functions} (AWAF).
%In what follows we will exploit the dimensional reduction afforded by HZD to obtain \emph{approximate walking arc functions} (AWAF) that can be computed efficiently while providing improved accuracy to the plan compared to NWA.
%Computing $\rho_p$ involves numerically integrating nonlinear dynamics which would slow down the planning process considerably. Previous work \cite{gregg-planning2012} dealt with this problem by admitting NWAs, $\mathcal{A}_p(z_p^*):=(\delta q_{1,p}(z_p^*),\delta X_p(z_p^*),\delta Y_p(z_p^*))$, as actions to the planner. 
% and change $(\delta X_p(z),\delta Y_p(z))$ in the CoM's Cartesian position over a stride depend only on $z$. The projection of the motion of the biped's CoM along the ground over a stride $(\delta X_p(z),\delta Y_p(z))$ .
%capture the evolution of the Cartesian position of the center of mass (CoM) and of the heading angle of the biped as it moves along a limit-cycle gait primitive ${\cal R}_p$. 
 

%basic actions in the form of \emph{nominal walking arcs} (NWAs) that are made available to the planning algorithm in its effort to construct paths that achieve desired specifications.  The NWAs capture the net change in the Cartesian position of the center of mass (CoM) and in the heading direction of the biped as it moves along a limit-cycle gait primitive ${\cal R}_p$. 
%We need more careful notation... For example, we define that a gait primitive is a fixed point and a Poincare map (like what Gregg has). But this only captures the discrete evolution of the system. The actual continuous evolution is the reduce-order hybrid system on $z$, which when integrated gives the reduced-order Poincare map. The Poincare map by itself does not provide any information on what happens along an arc. In this case, we should think of a better way to represent the gait primitives, which are limit cycles (the Poincare map is a tool to study existence and stability of a limit cycle, but if I only give you the Poincare map and a point, you will only be able to compute a bunch of other points which contain no information on what happens in between...)

%Thus, we can view $\delta q_{1,p}(z)$ and $(\delta X_p(z),\delta Y_p(z))$ as outputs of a discrete system whose dynamics are governed by \eqref{eq:zd-system}.   

%%In this section, we define \emph{nominal walking arcs} (NWA) made available to the planner as an action for constructing paths that achieve desired specifications, and discuss the drift accumulated while executing plans generated with NWA.
%
%To obtain the NWAs, we require the net change in the cartesian position of the center of mass (CoM), and the change in the heading direction, of the biped over a stride.
%%For planning motions in an environment cluttered by obstacles, it is of interest to obtain, the change in the center of mass (CoM) of the biped, and the change in its heading direction, over a stride. 
%According to \eqref{eq:decomp-poincare-z}, the change in heading angle, i.e. $\delta q_{1,p}$,  over a stride is dependent on $x$ only. The projection of the motion of the biped's CoM along the ground over a stride $(\delta X_p(z),\delta Y_p(z))$ expressed in a frame of reference attached to the stance toe and aligned in the current heading direction, is independent of $q_1$. Thus, we can view $\delta q_{1,p}(z)$ and $(\delta X_p(z),\delta Y_p(z))$ as outputs of a discrete system whose dynamics are governed by \eqref{eq:zd-system}.

%Hence, a gait primitive can be defined as a pair $\mathcal{G}_p=(\hat{P}_p,x^*_p)$. The primitive $\mathcal{G}_p$ is locally exponentially stable with respect to $x_p^*$ uniformly in $q_1$, if \eqref{eq:locomotion-specific} is locally exponentially stable with respect to $x_p^*$.


%Even though the evolution of the biped is governed by the corresponding Poincar\'e map $\rho_p$ and the associated outputs, 
%it is computationally infeasible to incorporate $\rho_p$ in the planner. 

%To achieve this, the planner would have to compute the Poincar\'e map for predicting the evolution of the state, as it works offline to generate \emph{a priori} motion plans.
% however, the caveat is that the planner would require the knowledge of $x$. It should be pointed out that the planner works offline to generate an \emph{a priori} motion plan which the biped executes, so feedback of $x$ is not possible while planning. Admitting the knowledge of $x$ to the planner at the beginning of each stride entails computing $P_p(x)$. 
%Hence, WAFs supplied to the planner are defined as $\mathcal{A}_p(z):=(\rho_p(z),\delta q_{1,p}(z),\delta X_p(z),\delta Y_p(z))$. 
%The lack of an analytical expression for $\rho_p(x)$ requires expensive numerical computations at each application of the primitive. 
%A primitive based on WAF is defined as $\mathcal{A}_p(z):=(\rho_p(z),\delta q_{1,p}^z(z),\delta \mathrm{cm}_p^z(z))$. The absence of analytical expressions makes numerical integration necessary which adversely affects planning speed. Hence, we will obtain approximate walking arc functions (AWAF) as our primitives for planning.
% by fitting polynomials to $\rho_p(z)$, $\delta q_{1,p}^z(z)$, and $\delta \mathrm{cm}_p^z(z)$.
%The functions of interest are 
%\begin{itemize}
%\item reduced order Poincar\'e map: $\rho_p(z)$,
%\item change in heading angle: $\delta q_{1,p}^z(z) = \rho_p^{q_1}(z)$, and
%\item change in the CoM measured in a frame aligned with the current heading direction: $\delta \mathrm{cm}_p^z(z)$.
%\end{itemize}
%All the above functions are smooth in $z$. 
%Note that $\delta \mathrm{cm}_p^z(z)$ has two components, $\delta \mathrm{cm}_{p,X}^z(z)$ and $\delta \mathrm{cm}_{p,Y}^z(z)$. 

 %We only note here that the dimensional reduction afforded by the HZD work on ${\cal S} \int {\cal Z}$
 %verification is performed using $V_p(z)$ to obtain positively invariant sublevel sets for applying Theorem~\ref{thm:switched}. 
 %rem
%\begin{rem}\label{rem:compact-set}
%As we are generating nominal plans, it is assumed that the initial state of \eqref{eq:zd-system} corresponds to a fixed point, i.e., $z[0]=z_p^*$ for some $p\in\mathcal{P}$. Hence, $z[0]\in\mathcal{N}(\kappa)\subset\underline{\mathcal{M}}(\kappa)$ for any $\kappa>0$. By applying Theorem~\ref{thm:switched} to the switched system \eqref{eq:zd-system} we obtain a dwell-time $N_{\rm d}$ which ensures stable execution of a plan. Additionally, Theorem~\ref{thm:switched} also guarantees evolution of \eqref{eq:zd-system} within the compact set $\overline{\mathcal{M}}(\kappa)$.
%\end{rem}
%%rem
